Combinatorial Register Allocation and Instruction Scheduling

This paper introduces a combinatorial optimization approach to register allocation and instruction scheduling, two central compiler problems. Combinatorial optimization has the potential to solve these problems optimally and to exploit processor-specific features readily. Our approach is the first to leverage this potential in practice: it captures the complete set of program transformations used in state-of-the-art compilers, scales to medium-sized functions of up to 1000 instructions, and generates executable code. This level of practicality is reached by using constraint programming, a particularly suitable combinatorial optimization technique. Unison, the implementation of our approach, is open source, used in industry, and integrated with the LLVM toolchain. An extensive evaluation confirms that Unison generates better code than LLVM while scaling to medium-sized functions. The evaluation uses systematically selected benchmarks from MediaBench and SPEC CPU2006 and different processor architectures (Hexagon, ARM, MIPS). Mean estimated speedup ranges from 1.1% to 10% and mean code size reduction ranges from 1.3% to 3.8% for the different architectures. A significant part of this improvement is due to the integrated nature of the approach. Executing the generated code on Hexagon confirms that the estimated speedup results in actual speedup. Given a fixed time limit, Unison solves optimally functions of up to 946 instructions, nearly an order of magnitude larger than previous approaches. The results show that our combinatorial approach can be applied in practice to trade compilation time for code quality beyond the usual compiler optimization levels, identify improvement opportunities in heuristic algorithms, and fully exploit processor-specific features.

==> figures/boundaries.tex <==
\newcommand{\drawCongruence}[8]{%
\begin{pgfonlayer}{layer0}
    \node [below=0cm of #1, block code] (pred) {\dots};
    \node [below=0cm of pred, block code] (post-pred) {%
      \begin{basicBlock}
        \alignCentered{\outOperation{#2}}
      \end{basicBlock}
    };
    \node [below=#8 of post-pred, block code] (pre-succ) {%
      \begin{basicBlock}
        \alignCentered{\inOperation{#3}}
      \end{basicBlock}
    };
    \node [below=0cm of pre-succ, block code] (succ) {\dots};
\end{pgfonlayer}
\begin{pgfonlayer}{main}
    % begin
    \node [cfg block filler, fit=(pred), minimum width=#5] (predDots) {};
    \node [cfg block boundary, fit=(post-pred), minimum width=#5] (post) {};
    \node [cfg boundary filler, below=0cm of post.north, minimum width=#5] {};

    % loop
    \node [cfg block boundary, fit=(pre-succ), minimum width=#5] (pre) {};
    \node [cfg boundary filler, above=0cm of pre.south, minimum width=#5] {};
    \node [cfg block filler, fit=(succ), minimum width=#5] {};

    \begin{scope}[flow]
      \draw (post) -- node[congruences, xshift=#6] (#1-congruences){%
        \begin{congruences}
          #4
        \end{congruences}
      } (pre);
    \end{scope}
    \ifstrequal{#7}{true}{%
      \begin{scope}[block label, left]
      \node at ([yshift=-0.2cm]predDots.north west) {\blockPredRaw{}:};
      \node at ([yshift=-0.2cm]pre.north west) {\blockSuccRaw{}:};
      \end{scope}}{}
\end{pgfonlayer}
}


==> figures/operations.tex <==
\newcommand{\drawOperation}[5][0.6cm]{%
  \coordinate [left=#1 of #2] (defs-#2);
  \coordinate [left=0cm of #2] (arrow-#2);
  \coordinate [right=0.5cm of #2] (uses-#2);
  \node [right=0cm of defs-#2, align=right, text width=0.43cm] (defs-math-#2) {#3};
  \node [right=0cm of arrow-#2] {#4};
  \node [right=0cm of uses-#2] (uses-math-#2) {#5};
}

\newcommand{\drawSimpleDefinerBeforeAfter}[1]{\drawOperation{#1}{$t$}{$\leftarrow$}{$\cdots$}}
\newcommand{\drawDefinerBeforeAfter}[1]{\drawOperation{#1}{$t$}{$\leftarrow$}{$i \,\cdots$}}
\newcommand{\drawUserBefore}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$t$}}
\newcommand{\drawVDots}[1]{\drawOperation{#1}{}{$\vdots$}{}}
\newcommand{\drawFirstUserAfter}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$\Operand{p}{\set{t,\Temp{1},\Temp{2},\ldots,\Temp{n}}}$}}
\newcommand{\drawUserAfter}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$\set{t,\Temp{1},\Temp{2},\ldots,\Temp{n}}$}}
\newcommand{\drawStoreAfter}[1]{\drawOperation{#1}{$\Temp{1}$}{$\leftarrow$}{$\set{\instruction{\genericStoreOpcode{}},\instruction{\genericMoveOpcode{}}} \,t$}}
\newcommand{\drawLoadAfter}[2]{\drawOperation{#1}{$\Temp{#2}$}{$\leftarrow$}{$\set{\instruction{\genericLoadOpcode{}},\instruction{\genericMoveOpcode{}}} \,\set{t,\Temp{1}}$}}
\newcommand{\drawDefinerDemat}[1]{\drawOperation{#1}{$t$}{$\leftarrow$}{$\set{i,\instruction{\genericDematOpcode{}}} \,\cdots$}}
\newcommand{\drawStoreDemat}[1]{\drawOperation{#1}{$\Temp{1}$}{$\leftarrow$}{$\set{\instruction{\genericStoreOpcode{}},\instruction{\genericMoveOpcode{}},\instruction{\genericDematOpcode{}}} \,t$}}
\newcommand{\drawLoadRemat}[2]{\drawOperation{#1}{$\Temp{#2}$}{$\leftarrow$}{$\set{\instruction{\genericLoadOpcode{}},\instruction{\genericMoveOpcode{}},i} \,\set{t,\Temp{1}}$}}

\newcommand{\drawFirstLoad}[1]{\drawOperation{#1}{$\Temp{1}$}{$\leftarrow$}{$\instruction{\armSingleLoad{}} \,t, n$}}
\newcommand{\drawSecondLoad}[1]{\drawOperation{#1}{$\Temp{2}$}{$\leftarrow$}{$\instruction{\armSingleLoad{}} \,t, n+4$}}
\newcommand{\drawFirstLoadUser}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$\Temp{1}$}}
\newcommand{\drawSecondLoadUser}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$\Temp{2}$}}
\newcommand{\drawDoubleLoad}[1]{\drawOperation[1.3cm]{#1}{$\Temp{1.d}, \Temp{2.d}$}{$\leftarrow$}{$\instruction{\armDoubleLoad{}} \,t, n$}}
\newcommand{\drawFirstLoadUserAfter}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$\set{\Temp{1},\Temp{1.d}}$}}
\newcommand{\drawSecondLoadUserAfter}[1]{\drawOperation{#1}{$\cdots$}{$\leftarrow$}{$\set{\Temp{2},\Temp{2.d}}$}}



==> figures/register-array.tex <==
\tikzset{%
  math mode/.style={%
    execute at begin node=$, execute at end node=$
  },
    cell/.style={%
      fill=white,
      minimum size=5.5mm,
      inner sep=0,
      outer sep=0,
      node distance=0,
    },
    border/.style={%
      draw,
      draw=gray,
      line width=0.2mm,
    },
    thick border/.style={%
      border,
      line width=0.25mm,
    },
    box/.style={%
      square,
      fill=white,
    },
    cycle/.style={%
      math mode
    },
    register/.style={%
    },
    label/.style={%
    },
    bundle/.style={%
      math mode,
    },
    braces/.style={%
      decorate,
      decoration={brace,amplitude=13pt},
      xshift=-4pt,
      line width=0.8mm
    },
}%

% Register array
\newcommand{\drawEmptyRegisterArray}[4][]{%
  \pgfmathtruncatemacro{\cycles}{#3}
  \pgfmathtruncatemacro{\regs}{#4}
  \coordinate [#1] (#2-c0-r1);
  \foreach \y in {1, ..., \cycles} {%
    \foreach \x in {1, ..., \regs} {%
      \pgfmathtruncatemacro{\prevY}{\y - 1}
      \pgfmathtruncatemacro{\prevX}{\x - 1}
      \ifnumequal{\x}{1}{%
        \node [cell, below=of #2-c\prevY-r\x] (#2-c\y-r\x) {};
      }{%
        \node [cell, right=of #2-c\y-r\prevX] (#2-c\y-r\x) {};
      }
    }
  }

  \foreach \y in {1, ..., \cycles} {%
    \pgfmathtruncatemacro{\yCycle}{\y - 1}
    \node [cycle, left= of #2-c\y-r1] (#2-c\y) {};
  }

  \begin{scope}[border]
    \foreach \x in {1, ..., \regs} {%
      \draw (#2-c1-r\x.north west) -- (#2-c\cycles-r\x.south west);
    }
    \draw (#2-c1-r\regs.north east) -- (#2-c\cycles-r\regs.south east);
    \foreach \y in {1, ..., \cycles} {%
      \draw (#2-c\y-r1.north west) -- (#2-c\y-r\regs.north east);
    }
    \draw (#2-c\cycles-r1.south west) -- (#2-c\cycles-r\regs.south east);
  \end{scope}
  \begin{scope}[thick border]
    \draw (#2-c1-r1.north west) -- (#2-c1-r\regs.north east) -- (#2-c\cycles-r\regs.south east)
          -- (#2-c\cycles-r1.south west) -- cycle;
  \end{scope}
}

\newcommand{\drawTemporary}[4][blockcolor]{%
  \node [box, fit=(#3) (#4)] {};
  \node [temporary box, fit=(#3) (#4), fill=#1] {\raisebox{-0.3cm}{$#2$}};
}

\newcommand{\drawBgTemporary}[4][boundarycolor]{%
  \node [box, fit=(#3) (#4)] {};
  \node [temporary box, fit=(#3) (#4), fill=#1, draw=gray] {\raisebox{-0.3cm}{\textcolor{gray}{$#2$}}};
}


==> figures/styles.tex <==

% Color definitions

\colorlet{blockcolor}{gray!30}
\colorlet{boundarycolor}{gray!20}

\colorlet{tempNColor}{gray!55}
\colorlet{tempAColor}{gray!32}
\colorlet{tempFColor}{gray!15}


% Dimensions and stuff

\newdimen\zerolinewidth%
\newdimen\cornerRadius%
\cornerRadius=3pt%

% TikZ styles

\tikzset{%
  invisible/.style={%
    draw opacity=0,
    fill opacity=0,
    text opacity=0,
  },
  file/.style={%
    inner sep=0.1cm,
    outer sep=0,
    node distance=2.7cm,
  },
  input/.style={%
    file,
  },
  output/.style={%
    file,
  },
  box/.style={%
    draw,
    line width=0.2mm,
    fill=white,
  },
  block/.style={%
    box,
    line width=0mm,
    inner sep=0cm,
    outer sep=0cm,
    rounded corners=\cornerRadius,
  },
  block code/.style={%
    inner sep=0cm,
    outer xsep=0cm,
    outer ysep=0.1cm,
    node distance=0
  },
  cfg block/.style={%
    block,
    fill=blockcolor,
    draw opacity=0,
  },
  cfg block boundary/.style={%
    block,
    fill=boundarycolor,
    draw opacity=0,
  },
  cfg block filler/.style={%
    cfg block,
    rounded corners=0mm,
    minimum height=0.3cm,
  },
  cfg boundary filler/.style={%
    cfg block boundary,
    rounded corners=0mm,
    minimum height=0.3cm,
  },
  line/.style={%
    -,
    line width=0.3mm,
  },
  live range/.style={%
    line,
    >=*,
    shorten <=-0.10515cm, shorten >=-0.10515cm,
  },
  copy/.style={%
    line,
    ->,
    >=stealth,
    shorten >= -0.017cm,
  },
  caption/.style={%
    font=\scriptsize,
  },
  flow/.style={%
    ->,
    >=stealth,
    line width=0.2mm,
  },
  secondary flow/.style={%
    ->,
    >=stealth,
    line width=0.2mm,
    dash pattern=on 1mm off 1mm,
  },
  block label/.style={%
    font=\it\footnotesize,
  },
  unison stage/.style={%
    cfg block,
    inner xsep=0.01cm,
    outer sep=0.05cm,
  },
  unison step/.style={%
    node distance=0cm,
    inner sep=0cm,
    outer sep=0cm,
  },
  square/.style={%
    fill=white,
    inner sep=0,
    outer sep=0,
    node distance=0,
  },
  temporary box/.style={%
    square,
    draw,
    line width=0.2mm,
  },
  congruences/.style={%
    font=\small,
  },
}


==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> results/arm-all-nocc-summary.tex <==
\newcommand{\noccARMAllNumberOfSolvedFunctions}{200}
\newcommand{\noccARMAllNumberOfBetterFunctions}{146}
\newcommand{\noccARMAllBest}{90.9}
\newcommand{\noccARMAllNumberOfWorseFunctions}{0}
\newcommand{\noccARMAllWorst}{-0}
\newcommand{\noccARMAllMeanImprovement}{12.3}
\newcommand{\noccARMAllNumberOptimal}{133}
\newcommand{\noccARMAllPercentOptimal}{66.5}
\newcommand{\noccARMAllMeanGap}{7.2}
\newcommand{\noccARMAllMeanNonZeroGap}{23.1}
\newcommand{\noccARMAllMeanNonZeroSmallGap}{24.6}
\newcommand{\noccARMAllMeanNonZeroLargeGap}{14.9}
\newcommand{\noccARMAllLargestOptimalIns}{360}
\newcommand{\noccARMAllSmallestNonZeroGapIns}{55}
\newcommand{\noccARMAllPercentGecodeSolverTotal}{51.9}
\newcommand{\noccARMAllLargestGecodeWin}{748}
\newcommand{\noccARMAllLargestMinizincWin}{664}
\newcommand{\noccARMAllGecodeAboveMinizinc}{1}
\newcommand{\noccARMAllMedianNonZeroGapIns}{226}
\newcommand{\noccARMAllTenPercentNonZeroGapIns}{182}
\newcommand{\noccARMAllMeanInitialGap}{21.7}
\newcommand{\noccARMAllMeanSpillNumberImprovement}{12.3}
\newcommand{\noccARMAllMeanSpillNumberWorsening}{-12.3}
\newcommand{\noccARMAllMeanSpillOverheadImprovement}{-589.3}
\newcommand{\noccARMAllMeanSpillOverheadWorsening}{589.3}


==> results/arm-all-unitlatency-summary.tex <==
\newcommand{\unitlatencyARMAllNumberOfSolvedFunctions}{200}
\newcommand{\unitlatencyARMAllNumberOfBetterFunctions}{105}
\newcommand{\unitlatencyARMAllBest}{42.9}
\newcommand{\unitlatencyARMAllNumberOfWorseFunctions}{0}
\newcommand{\unitlatencyARMAllWorst}{-0}
\newcommand{\unitlatencyARMAllMeanImprovement}{3.1}
\newcommand{\unitlatencyARMAllNumberOptimal}{125}
\newcommand{\unitlatencyARMAllPercentOptimal}{62.5}
\newcommand{\unitlatencyARMAllMeanGap}{6.4}
\newcommand{\unitlatencyARMAllMeanNonZeroGap}{18.1}
\newcommand{\unitlatencyARMAllMeanNonZeroSmallGap}{18.8}
\newcommand{\unitlatencyARMAllMeanNonZeroLargeGap}{13.5}
\newcommand{\unitlatencyARMAllLargestOptimalIns}{330}
\newcommand{\unitlatencyARMAllSmallestNonZeroGapIns}{55}
\newcommand{\unitlatencyARMAllPercentGecodeSolverTotal}{52.9}
\newcommand{\unitlatencyARMAllLargestGecodeWin}{513}
\newcommand{\unitlatencyARMAllLargestMinizincWin}{748}
\newcommand{\unitlatencyARMAllGecodeAboveMinizinc}{0}
\newcommand{\unitlatencyARMAllMedianNonZeroGapIns}{222}
\newcommand{\unitlatencyARMAllTenPercentNonZeroGapIns}{158}
\newcommand{\unitlatencyARMAllMeanInitialGap}{12.5}
\newcommand{\unitlatencyARMAllMeanSpillNumberImprovement}{8.5}
\newcommand{\unitlatencyARMAllMeanSpillNumberWorsening}{-8.5}
\newcommand{\unitlatencyARMAllMeanSpillOverheadImprovement}{-37.2}
\newcommand{\unitlatencyARMAllMeanSpillOverheadWorsening}{37.2}


==> results/hexagon-all-nocc-summary.tex <==
\newcommand{\noccHexagonAllNumberOfSolvedFunctions}{200}
\newcommand{\noccHexagonAllNumberOfBetterFunctions}{117}
\newcommand{\noccHexagonAllBest}{138.9}
\newcommand{\noccHexagonAllNumberOfWorseFunctions}{0}
\newcommand{\noccHexagonAllWorst}{-0}
\newcommand{\noccHexagonAllMeanImprovement}{11.8}
\newcommand{\noccHexagonAllNumberOptimal}{165}
\newcommand{\noccHexagonAllPercentOptimal}{82.5}
\newcommand{\noccHexagonAllMeanGap}{1.9}
\newcommand{\noccHexagonAllMeanNonZeroGap}{13.7}
\newcommand{\noccHexagonAllMeanNonZeroSmallGap}{16.8}
\newcommand{\noccHexagonAllMeanNonZeroLargeGap}{7}
\newcommand{\noccHexagonAllLargestOptimalIns}{647}
\newcommand{\noccHexagonAllSmallestNonZeroGapIns}{64}
\newcommand{\noccHexagonAllPercentGecodeSolverTotal}{65.9}
\newcommand{\noccHexagonAllLargestGecodeWin}{946}
\newcommand{\noccHexagonAllLargestMinizincWin}{613}
\newcommand{\noccHexagonAllGecodeAboveMinizinc}{6}
\newcommand{\noccHexagonAllMedianNonZeroGapIns}{419}
\newcommand{\noccHexagonAllTenPercentNonZeroGapIns}{456}
\newcommand{\noccHexagonAllMeanInitialGap}{11}
\newcommand{\noccHexagonAllMeanSpillNumberImprovement}{33.1}
\newcommand{\noccHexagonAllMeanSpillNumberWorsening}{-33.1}
\newcommand{\noccHexagonAllMeanSpillOverheadImprovement}{272.7}
\newcommand{\noccHexagonAllMeanSpillOverheadWorsening}{-272.7}


==> results/hexagon-all-unitlatency-summary.tex <==
\newcommand{\unitlatencyHexagonAllNumberOfSolvedFunctions}{200}
\newcommand{\unitlatencyHexagonAllNumberOfBetterFunctions}{72}
\newcommand{\unitlatencyHexagonAllBest}{95.5}
\newcommand{\unitlatencyHexagonAllNumberOfWorseFunctions}{0}
\newcommand{\unitlatencyHexagonAllWorst}{-0}
\newcommand{\unitlatencyHexagonAllMeanImprovement}{5.4}
\newcommand{\unitlatencyHexagonAllNumberOptimal}{157}
\newcommand{\unitlatencyHexagonAllPercentOptimal}{78.5}
\newcommand{\unitlatencyHexagonAllMeanGap}{3.4}
\newcommand{\unitlatencyHexagonAllMeanNonZeroGap}{17.4}
\newcommand{\unitlatencyHexagonAllMeanNonZeroSmallGap}{18}
\newcommand{\unitlatencyHexagonAllMeanNonZeroLargeGap}{14.9}
\newcommand{\unitlatencyHexagonAllLargestOptimalIns}{946}
\newcommand{\unitlatencyHexagonAllSmallestNonZeroGapIns}{101}
\newcommand{\unitlatencyHexagonAllPercentGecodeSolverTotal}{58.8}
\newcommand{\unitlatencyHexagonAllLargestGecodeWin}{946}
\newcommand{\unitlatencyHexagonAllLargestMinizincWin}{874}
\newcommand{\unitlatencyHexagonAllGecodeAboveMinizinc}{1}
\newcommand{\unitlatencyHexagonAllMedianNonZeroGapIns}{277}
\newcommand{\unitlatencyHexagonAllTenPercentNonZeroGapIns}{271}
\newcommand{\unitlatencyHexagonAllMeanInitialGap}{9.3}
\newcommand{\unitlatencyHexagonAllMeanSpillNumberImprovement}{-15.4}
\newcommand{\unitlatencyHexagonAllMeanSpillNumberWorsening}{15.4}
\newcommand{\unitlatencyHexagonAllMeanSpillOverheadImprovement}{-43.4}
\newcommand{\unitlatencyHexagonAllMeanSpillOverheadWorsening}{43.4}


==> results/mips-all-nocc-summary.tex <==
\newcommand{\noccMipsAllNumberOfSolvedFunctions}{200}
\newcommand{\noccMipsAllNumberOfBetterFunctions}{160}
\newcommand{\noccMipsAllBest}{150}
\newcommand{\noccMipsAllNumberOfWorseFunctions}{0}
\newcommand{\noccMipsAllWorst}{-0}
\newcommand{\noccMipsAllMeanImprovement}{26.6}
\newcommand{\noccMipsAllNumberOptimal}{144}
\newcommand{\noccMipsAllPercentOptimal}{72}
\newcommand{\noccMipsAllMeanGap}{6.5}
\newcommand{\noccMipsAllMeanNonZeroGap}{26.3}
\newcommand{\noccMipsAllMeanNonZeroSmallGap}{25.8}
\newcommand{\noccMipsAllMeanNonZeroLargeGap}{27.8}
\newcommand{\noccMipsAllLargestOptimalIns}{403}
\newcommand{\noccMipsAllSmallestNonZeroGapIns}{78}
\newcommand{\noccMipsAllPercentGecodeSolverTotal}{43.3}
\newcommand{\noccMipsAllLargestGecodeWin}{577}
\newcommand{\noccMipsAllLargestMinizincWin}{812}
\newcommand{\noccMipsAllGecodeAboveMinizinc}{0}
\newcommand{\noccMipsAllMedianNonZeroGapIns}{307}
\newcommand{\noccMipsAllTenPercentNonZeroGapIns}{223}
\newcommand{\noccMipsAllMeanInitialGap}{29.5}
\newcommand{\noccMipsAllMeanSpillNumberImprovement}{41.3}
\newcommand{\noccMipsAllMeanSpillNumberWorsening}{-41.3}
\newcommand{\noccMipsAllMeanSpillOverheadImprovement}{279.3}
\newcommand{\noccMipsAllMeanSpillOverheadWorsening}{-279.3}


==> results/mips-all-unitlatency-summary.tex <==
\newcommand{\unitlatencyMipsAllNumberOfSolvedFunctions}{200}
\newcommand{\unitlatencyMipsAllNumberOfBetterFunctions}{99}
\newcommand{\unitlatencyMipsAllBest}{90.2}
\newcommand{\unitlatencyMipsAllNumberOfWorseFunctions}{0}
\newcommand{\unitlatencyMipsAllWorst}{-0}
\newcommand{\unitlatencyMipsAllMeanImprovement}{6.6}
\newcommand{\unitlatencyMipsAllNumberOptimal}{115}
\newcommand{\unitlatencyMipsAllPercentOptimal}{57.5}
\newcommand{\unitlatencyMipsAllMeanGap}{8.9}
\newcommand{\unitlatencyMipsAllMeanNonZeroGap}{22.5}
\newcommand{\unitlatencyMipsAllMeanNonZeroSmallGap}{22.5}
\newcommand{\unitlatencyMipsAllMeanNonZeroLargeGap}{22.1}
\newcommand{\unitlatencyMipsAllLargestOptimalIns}{324}
\newcommand{\unitlatencyMipsAllSmallestNonZeroGapIns}{39}
\newcommand{\unitlatencyMipsAllPercentGecodeSolverTotal}{44.7}
\newcommand{\unitlatencyMipsAllLargestGecodeWin}{403}
\newcommand{\unitlatencyMipsAllLargestMinizincWin}{812}
\newcommand{\unitlatencyMipsAllGecodeAboveMinizinc}{0}
\newcommand{\unitlatencyMipsAllMedianNonZeroGapIns}{215}
\newcommand{\unitlatencyMipsAllTenPercentNonZeroGapIns}{112}
\newcommand{\unitlatencyMipsAllMeanInitialGap}{19.8}
\newcommand{\unitlatencyMipsAllMeanSpillNumberImprovement}{-15.1}
\newcommand{\unitlatencyMipsAllMeanSpillNumberWorsening}{15.1}
\newcommand{\unitlatencyMipsAllMeanSpillOverheadImprovement}{12.6}
\newcommand{\unitlatencyMipsAllMeanSpillOverheadWorsening}{-12.6}


==> results/single-issue-all-summary.tex <==
\newcommand{\singleissueHexagonAllNumberOfSolvedFunctions}{200}
\newcommand{\singleissueHexagonAllNumberOfBetterFunctions}{30}
\newcommand{\singleissueHexagonAllBest}{37.3}
\newcommand{\singleissueHexagonAllNumberOfWorseFunctions}{3}
\newcommand{\singleissueHexagonAllWorst}{-2}
\newcommand{\singleissueHexagonAllMeanImprovement}{1.5}
\newcommand{\singleissueHexagonAllNumberOptimal}{170}
\newcommand{\singleissueHexagonAllPercentOptimal}{85}
\newcommand{\singleissueHexagonAllMeanGap}{3.4}
\newcommand{\singleissueHexagonAllMeanNonZeroGap}{24.9}
\newcommand{\singleissueHexagonAllMeanNonZeroSmallGap}{27.2}
\newcommand{\singleissueHexagonAllMeanNonZeroLargeGap}{16.1}
\newcommand{\singleissueHexagonAllLargestOptimalIns}{946}
\newcommand{\singleissueHexagonAllSmallestNonZeroGapIns}{64}
\newcommand{\singleissueHexagonAllPercentGecodeSolverTotal}{78.8}
\newcommand{\singleissueHexagonAllLargestGecodeWin}{946}
\newcommand{\singleissueHexagonAllLargestMinizincWin}{874}
\newcommand{\singleissueHexagonAllGecodeAboveMinizinc}{2}
\newcommand{\singleissueHexagonAllMedianNonZeroGapIns}{228}
\newcommand{\singleissueHexagonAllTenPercentNonZeroGapIns}{278}
\newcommand{\singleissueHexagonAllMeanInitialGap}{21}
\newcommand{\singleissueHexagonAllMeanSpillNumberImprovement}{-3.9}
\newcommand{\singleissueHexagonAllMeanSpillNumberWorsening}{3.9}
\newcommand{\singleissueHexagonAllMeanSpillOverheadImprovement}{-7.6}
\newcommand{\singleissueHexagonAllMeanSpillOverheadWorsening}{7.6}

